Not All Errors are Equal: Learning Text Generation Metrics using Stratified Error Synthesis

Is it possible to build a general and automatic natural language generation (NLG) evaluation metric? Existing learned metrics either perform unsatisfactorily or are restricted to tasks where large human rating data is already available. We introduce SESCORE, a model-based metric that is highly correlated with human judgements without requiring human annotation, by utilizing a novel, iterative error synthesis and severity scoring pipeline. This pipeline applies a series of plausible errors to raw text and assigns severity labels by simulating human judgements with entailment. We evaluate SESCORE against existing metrics by comparing how their scores correlate with human ratings. SESCORE outperforms all prior unsupervised metrics on multiple diverse NLG tasks including machine translation, image captioning, and WebNLG text generation. For WMT 20/21 En-De and Zh-En, SESCORE improve the average Kendall correlation with human judgement from 0.154 to 0.195. SESCORE even achieves comparable performance to the best supervised metric COMET, despite receiving no human-annotated training data.

==> sections/03noise_formulation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.65\linewidth]{figures/model.pdf}
    \caption{Overview of the Quality Prediction Model}
    \label{fig:model}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=.98\linewidth]{figures/SEScore.pdf}
    \caption{Stratified Error Synthesis and Severity Scoring Pipeline. Red Cross indicates the start index of each error in the previous sentence. Both MLM or Seq-to-seq models can be used to produce inserted or replaced tokens. The above example has final score of -12}
    \label{fig:method}
\end{figure*}

% \subsection{Problem Formulation}
Given a reference sentence $x$ and a candidate $y$, our goal is to train a model $f(\theta)$ to predict the quality of $y$ against $x$.
Such reference-based metric does not require source input, therefore it is applicable to diverse text generation tasks including open-end generation, machine translation, etc. 
Ideally, training such a model needs triples of $\{\langle x, y, s \rangle\}$ where $s$'s are human ratings. 
However, such human ratings are usually available for evaluation but not for training. 
We present a method to pre-train such a metric without relying on human ratings of reference-candidate pairs.  




\subsection{The Overall Pretraining Framework}

% Yi-Lin: should the pair be $\{(x,y),s\}$ or $\{(x^i,y^i),s^i\}$ for sentence-level score?

%  Due to the scarcity of the human labeled output candidates, a large scale $\{(x_i, y_i), s_i\}$ pairs are unavailable to enable supervised training in many domains and tasks.
During the pre-training, given raw sentences, we create a synthetic triplet set with simulated candidate text and estimated ratings. 
We train the metric using the synthetic data, shown in Figure \ref{fig:model}. 


To this end, we construct a stratified error synthesis function, $f_{ses}$. 
It takes a raw sentence $x_{raw}$ and outputs a perturbed sentence $y_i$ to mimic text errors.
% Yi-Lin: How about changing the "candidate text generation result" to "hypothesis candidates"?
Within the stratified error synthesis function, $f_{ses}$, we define a set of error function types based on plausible errors in text generation, $E=\{e1, e2, ..., e_k\}$.
For each raw text instance, $x_{raw}$, we randomly draw a subset of error signals in $E$ and iteratively edit the text accordingly.
At each iteration, we estimate the severity level of the created error and assign a negative score accordingly.
After completing all the steps in one instance, we obtained the final score by summing the scores assigned at all prior steps, shown in Figure \ref{fig:method}. 
% Yi-Lin: how many steps

Therefore, given a set of raw texts, our stratified error synthesis function, $f_{ses}$, can synthesize a dataset with triplets, $\{\langle x_i, y_i, s_i\rangle\}$, while $y_i$ is the synthesized candidate sentence and $s_i$ is the severity rating indicating the quality of the candidate sentence compared to the reference. Therefore, only given a set of raw input text $\{x_i\}$, our pretraining pipeline can learn a function $f_{ses}$ to map the embeddings of ${x_i, y_i}$ pairs to a quality score $s_i$.

\begin{table*}
  \label{langtable}
  \centering
  \small
  \resizebox{\textwidth}{!}{
  \begin{tabular}{llll}
    \toprule
    Category &  & MQM Description & Synthesis Procedure in \method\\
    \midrule
    Accuracy & Addition & Text includes information not present reference. & insertion using masked or seq2seq generation\\
    & Omission & Text is missing content from the reference & Deletion a random span of tokens \\
    & Mistranslation & Text does not accurately represent the reference & Replacement a random span using maksed or seq2seq generation \\
    Fluency & Punctuation & Incorrect punctuation (for locale or style) & Insertion \& replacement using masked filling, and deletion \\
    & Spelling & Incorrect spelling or capitalization &  
    Insertion, replacement, deletion, and Swap\\
    & Grammar & Problems with grammar & Insertion, replacement, deletion, and Swap \\
    \bottomrule
  \end{tabular}
    }
    \caption{
    Error Categories in MQM and our synthesis procedure. \method generalize the imitate human errors beyond machine translation.   % \yj{name for the second column?}
    }
  \label{tab:error_type}
\end{table*}

\subsection{Background: Quality Measured by Errors}
Our method is inspired by the human evaluation procedure for machine translation.
The multidimensional quality metrics (MQM) determine the quality of a translation text by labelling errors and their severity levels~\cite{freitag2021experts}. 
Errors are categorized into multiple types such as accuracy and fluency. 
Within each type, an error has an associated severity level -- a penalty of 5 for major error and 1 for minor error. 


Inspired by the MQM's success in human evaluation, we use its two major error categories, accuracy and fluency, to classify and decide our synthetic error types in $f_{ses}$.
In Table \ref{tab:error_type}, we demonstrate accuracy and fluency with their subcategories and  descriptions.
There are two main motivations to simulate those errors from the table: 1) they are two major error categories in machine translations; 2) those errors are general and can be extensible to new domains. We use six techniques to simulate errors from the Table \ref{tab:error_type}:
mask insertion/replacement with maksed language mode/sequence-to-sequence language model, and N-gram word drop/swap. 



\subsection{Stratified Error Synthesis}
As prior study \citet{freitag2021experts,tuan2021quality} suggested that multiple errors could co-occur in one segment, we construct each sentence with up to $\lambda_e$ editing operations ($\lambda_e=5$ in experiments). 
Since we require stratified generation to evaluate severity at each iteration, the creation of each error has to take the consideration of all the prior steps.
In particular, we do not want posterior pseudo errors to modify or overwrite the prior ones.

To handle the above issue, we propose a novel stratified error synthesis algorithm. For a given sentence input $x$, with $k$ tokens, we initialize an array $q$ of length $k$, with values of $k-1, k-2, ..., 0$. Values indicate the number of tokens after the current token can be modified with the error signal. Each error signal will randomly select a start index $j$ from $1$ to $k$.
We define an error synthesis table to keep track of the number of candidate tokens can be modified at after index $j$. The error signal will only be accepted if $q_j$ is greater than the span length of the error signal. The specific stratified error synthesis algorithm regarding to each error type is illustrated in Algorithm \ref{alg:SSE}.

\begin{algorithm}\small
  \caption{Stratified Error Synthesis \yj{need some simplification here, e.g. move the common sampling part before switch-case statement}}
  \label{alg:SSE}
  \KwIn{Seed sentence set $S = \{x_1, x_2, ... , x_n\}$, $\lambda_e$, $\lambda_d$, $\lambda_r$, $\lambda_s$, editing model set $M$.}
  \KwOut{Synthetic reference and error text $D$.}
%   $\sum_{1}^{n} (\{(x_i, y'_i ), s'_i\})$, where $y_i$ is synthesized error sentence and $s'_i$ is the pseudo rating
  $D=\emptyset$\;
  \For{$i = 1 .. n$}{
    $l = len(x_i)$, 
    $y_{new} = x_i$, $s_i=0$\;
    $k \sim Poisson(\lambda_e)$\; 
    \For{$j = 1 .. k$}{
        $y_{\text{old}}=y_{\text{new}}$\;
        $\mathrm{edit} \sim \mathrm{Random}(\{\mathrm{Ins}, \mathrm{Del}, \mathrm{Rep}, \mathrm{Swap}\})$\;
        \Switch{$\mathrm{edit}$}{
            \Case{\textup{Ins}}{
                sampling $h \sim \mathrm{Uniform}(0, l)$ s.t. $h$ does not overlap the previous edited spans\;
                Randomly select a model from $M$ to generate a phrase $f$ to insert at position $h$ of $y_{\text{new}}$\;
            }
            \Case{\textup{Del}}{
                \Repeat{the span from $h$ to $b+ll-1$ does not overlap the previous edited spans}{
                    draw $h \sim \mathrm{Uniform}(0,l)$\;
                    draw $ll \sim \mathrm{Poisson}(\lambda_d)$\;
                }
                Remove a span of length $ll$ at position $h$ from  $y_{\text{new}}$\;
            }
            \Case{\textup{Rep}}{
                \Repeat{the span from $h$ to $b+ll-1$ does not overlap the previous edited spans}{
                    draw $h \sim \mathrm{Uniform}(0,l)$\;
                    draw $ll \sim \mathrm{Poisson}(\lambda_r)$\;
                }
                Randomly select a model from the model base $M$ to generate a phrase $f$\;
                Replace the segment of $y_{\text{new}}$ from $h$ to $h+ll-1$ with $f$\;
            }
            \Case{\textup{Swap}}{
                \Repeat{the span from $b$ to $b+ll-1$ does not overlap the previous edited spans}{
                    draw $h \sim \mathrm{Uniform}(0,l)$\;
                    draw $ll \sim \mathrm{Uniform}(1..\lambda_s)$\;
                }
                Swap the tokens in $y_{\text{new}}$ at positions $h$ and $h+ll$\;
            }
        }
        $s_i += \text{SeverityScore}(y_{old}, y_{new})$\;
    }
    $D \leftarrow D \cup \{(x_i, y_{new}, s_i) \}$\;
  }
%     Initialize an array $q_i$ with length $k$ and values of $k-1, k-2, ..., 0$ \\
%     Draw a Possion distribution $\lambda=1.5$ from 1 to 5 for the number of error iterations on $x_i$ \\
%     \For{each iteration of text $x_i$}
%     {
%         Randomly select an error function, $f_{es}$ from $insert$, $replace$, $delete$ and $swap$ \\
%         Randomly select a start index from tokenized length, $j$ \\
%         \If{$f_{es} == insert$ and $q_i[j] > 0$} {
%             Insert a $<mask>$ token after j \\
%             Use MBart or Roberta to predict the $<mask>$ \\ 
%             update all tokens on the left of j with $min(j-1, k-1)$
%         } 
%     }
%   }
 \end{algorithm}



\paragraph{Synthesize addition error by insertion}
Given an index, we add additional phrase in the reference sentence with
two ways: a) using a masked language model (e.g. BERT and RoBERTa), and b) using a sequence-to-sequence language model (e.g. mBART). 

For the first approach, we insert a \verb|<mask>| token at the given position of a sentence.
We then use a maksed language model to fill the token based on its context. 
We use top-k sampling, with k=4, to randomly select the filling token.
Many of those <mask>s are randomly placed within the word.
% Yi-Lin: "a" word
Our primary aim is to introduce the semantically close sentences with all three fluency errors. 
With insertion of <mask>, we can further synthesize the Addition errors.

For the second approach, we use a pre-trained sequence-to-sequence model (e.g. mBART) to generate a phrase given the context text. 
In this case, it will generate insertion phrases with variable length. 

% Mask Insertion and Replacement with Roberta\ww{Be consistent with spelling and capitalization. Consult original paper for capitalization.}.



% RoBERTa's mask infilling objective enables the model to predict on the <mask> token at its left and right context.
% \ww{I'm not sure if we should name a specific in-filling model like RoBERTa in this approach section: imagine if 5 years later, no one is using RoBERTa anymore, but your paper can still be relevant, and people can use other in-filling LMs, correct?}
% Yi-Lin: what does "on the <mask> token at its left and right context" mean?

% Yi-Lin: how does insertion and replacement can be applied in the same time?

\paragraph{Synthesize omission by deletion.}
We drop a random span of tokens in a raw text sentence. 
The position of the span is drawn uniformly within sentence. 
The length of the span is drawn from a Poisson distribution with the parameter $\lambda_d$ (=1.5 in experiment).
Our primary aim is to mimic omission error in the Accuracy. However, depending on the specific words that it drops. This technique can further create mistranslation and all fluency errors. 



\paragraph{Synthesize phrasal error by replacement.}
While comparing difference between the reference text and a candidate sentence, certain phrase can be erroneous. 
This is difficult to simulate. 
Instead, we use either a masked language model or a sequence-to-sequence model to replace a segment of tokens in the original text. 

For the first approach, the replaced span is always one single token. 
We  replace a random token from the original text with one \verb|<mask>| token. 
We then use a masked language model to fill the blank similar to the insertion operation. 

For the second approach, we use a denoising sequence-to-sequence model (e.g. mBART) to generate the tokens for the mask tags. 
We randomly choose the starting index of the span and draw the span length from a Poisson distribution with parameter $\lambda_r$ (=1.5 in experiments).
We use a denoising sequence-to-sequence model like mBART to synthesize fluent sentences with \emph{Addition} and \emph{Mistranslation} errors. Through the model's rewriting capability, we can dynamically modify sentence length through injected error locations.  

% Different from Roberta's mask infilling objective, MBart predicts a span of tokens for its <mask> position through auto-regressive rewriting. We leverage this functionality by inserting and replacing a span of tokens in the raw text though MBart. We draw a possion distribution with $\lambda=1.5$ to determine the replaced span length. Since MBart is trained as a denoising autoencoder, We expect this rewriting to produce fluent sentences but introducing 'Addition' and 'Mistranslation' errors. Through MBart's rewriting, we can dynamically modify sentence length through injected error locations.  


\paragraph{Synthesize grammar and other errors by swapping.}
We swap random two words within the span length of $\lambda_s$ in the sentence. Our primary aim is to generate grammatically incorrect sentences with mismanagement of word orders, such as subject verb disagreement. It further introduces spelling and punctuation errors.
We set $\lambda_s=4$ in our implementation.


\subsection{Severity Scoring}
As suggested by the recent work \cite{freitag2021experts}, different errors in the sentence can have different severity measures, depending on the level that they mislead the readers.
Following the definition, we define the severe error as if the error alter the semantic meaning of the sentence.
Prior study has suggested that sentence entailment has strong correlation to the semantic similarities \cite{khobragade2019machine}.
To capture the change of semantic meaning, we further define a bidirectional entailment relation such that, $a$ entails $b$ and $b$ entails $a$ is equivalent to $a$ is semantically equivalent to $b$.
Therefore, for a given noise signal $e_i$ on the sentence $x$, we measure a bidirectional entailment likelihood of $x'$ and $x$.
If after applying noises on $x$, $x'$ remains bidirectional entailed to $x$, we can assume that error $e_i$ does not severely alter the original semantic meaning of $x$ and therefore it is a minor error.
We choose XLM-Roberta large model which pretrained on multi-lingual natural language inference datasets as our entailment likelihood estimator.
We define the entailment likelihood as the probability of predicting entailment class.
We evaluate entailments in both $x \rightarrow x'$ and $x'\rightarrow x$ directions.
According to our validation dataset, setting the threshold, $\theta$ of 0.9 reaches the highest inter-rater agreement on the severity measures.
Therefore, $p_{mnli}(x\rightarrow x')$ and $p_{mnli}(x'\rightarrow x)$ have to be both greater than 0.9.
Following the MQM severity labels, we give -5 to severe error and -1 to minor errors. Therefore, our range of score is between -25 to 0.
%  Yi-Lin: change p_{mnli} -> \rho
% \yj{0.9=>threshold $\theta$}
\begin{align*}
        & \text{SeverityScore}(x,x')=\\
        & \begin{cases}
    -1, & \text{if } \rho_{x\rightarrow x'} \geq  \theta \text{ and }\rho_{x'\rightarrow x} \geq \theta\\
    -5, & \text{ otherwise}
    \end{cases}
        %& \left\{\right .
\end{align*}

\iffalse
\[
    SeverityScore(x, x')= 
    \begin{cases}
    -1, & \text{if } $p_{mnli}(x->x') \geq  0.9$ and $p_{mnli}(x'->x) \geq 0.9$\\
    -5, & \text{$Otherwise$}
    \end{cases}
\]
\fi
% We synthesize data from the News Complimentary datasets. For each instance, we create candidate pseudo output sentences using six different noise functions. Each noise is applied iteratively with the maximum iteration to be 5. We draw a Possion distribution ($\lambda=1.5$) to determine the number of noises applied to each instance.  

%For each step, one of the six noise functions will be randomly selected and applied to a random positions of the sentence. After the pseudo output sentence is generated at each step, We use a classification model to determine error's severity. Each error will be given either score of -1 or -5, based on its severity measure. After all the error steps completed on each sentence, we obtain a pseudo sentence quality rating based on all prior severity measures. Based on the prior study \cite{freitag2021experts}, 

\subsection{Quality Prediction Model}
 In Figure \ref{fig:model}, similar to the COMET configuration \cite{rei-etal-2020-comet}, we fed both reference sentence and candidate sentence into the pretrained language model. The resulting word embeddings are average  pooled to derive the two sentence embeddings, $h$ and $f$, $h$ is our synthesized error sentence and $f$ is the raw text sentence. With the sentence embeddings of the two, we use the approach proposed by RUSE \cite{shimanaka-etal-2018-ruse} to extract the two features: 
\begin{itemize}
    \item Element-wise synthesize error sentence and raw sentence product 
    % \yj{incomplete sentence}
   \item Element-wise synthesize error sentence and raw sentence difference
\end{itemize}

Following the COMET \cite{rei-etal-2020-comet} implementation, two features are concatenated into a single vector and feed into a feedward neural network regressor. However, the key distinction between our model and COMET is that we don't use source sentence during training or inference. Therefore, we do not need parallel text sentences for the evaluation metric. The detailed architecture choice and analysis can be found in Sect. 








